HAT-P-54b: A hot jupiter transiting a 0.64 Msun star in field 0 of the K2 mission

We report the discovery of HAT-P-54b, a planet transiting a late K dwarf star in field 0 of the NASA K2 mission. We combine ground-based photometric light curves with radial velocity measurements to determine the physical parameters of the system. HAT-P-54b has a mass of 0.760 $\pm$ 0.032 $M_J$, a radius of 0.944 $\pm$ 0.028 $R_J$, and an orbital period of 3.7998 d. The star has V = 13.505 $\pm$ 0.060, a mass of 0.645 $\pm$ 0.020 $M_{\odot}$, a radius of 0.617 $\pm$ 0.013 $R_{\odot}$, an effective temperature of Teff = 4390 $\pm$ 50K, and a subsolar metallicity of [Fe/H] = -0.127 $\pm$ 0.080. HAT-P-54b has a radius that is smaller than 92% of the known transiting planets with masses greater than that of Saturn, while HAT-P-54 is one of the lowest-mass stars known to host a hot Jupiter. Follow-up high-precision photometric observations by the K2 mission promise to make this a well-studied planetary system.

==> makefile <==
TARGET=ms
PRINTER=peyton_color
SUB=submit_v1
CURRENTDIR=$(shell pwd | sed -e 's|.*/||g')
VERSION=$(shell ls -l $(TARGET).tex | \
	sed -e 's|.*->||g' -e 's|.*_V||g' -e 's|.tex||g')
VERSION=07

all: $(TARGET).pdf

.PHONY: all clean save print show


show:
	@echo VERSION: $(VERSION)

#$(TARGET).dvi: *.tex *.cls *.bib
$(TARGET).dvi: *.tex *.bib
	#sed -e "s|HATVERSION|$(VERSION)|g" emulateapj_template.cls > emulateapj.cls
	latex $(TARGET).tex
	latex $(TARGET).tex
	bibtex $(TARGET)
	latex $(TARGET).tex
	latex $(TARGET).tex
	latex $(TARGET).tex

$(TARGET).ps: $(TARGET).dvi
	dvips -t letter $(TARGET).dvi -o

$(TARGET).pdf: $(TARGET).ps
	ps2pdf $< $@

save:
	tar cvzf ../$(TARGET)_V$(VERSION).tgz ../$(CURRENTDIR)/
	#gzip $(TARGET).tar
	#mv $(TARGET).tar.gz $(TARGET).tgz

sub:
	test -d $(SUB) || mkdir $(SUB)
	test -d $(SUB)/img || mkdir $(SUB)/img
	cp $(TARGET).tex $(SUB)/hatpxx.tex
	cp img/*.eps $(SUB)/img

clean:
	rm -f $(TARGET).ps \
	$(TARGET).dvi \
	$(TARGET).aux \
	$(TARGET).log \
	$(TARGET).pdf \
	$(TARGET).idx \
	$(TARGET).inx \
	$(TARGET).toc \
	$(TARGET).tgz
	
print: $(TARGET).ps
	lpr -P$(PRINTER) $<
	

